Precise Predictions for $\mu^{\pm}e^-\rightarrow\mu^{\pm}e^-$ at the MUonE Experiment

The proposed fixed-target experiment, MUonE, at CERN will aim to measure the hadronic contribution to the running of the QED coupling by analysing the scattering of muons on electrons. Here we present state-of-the-art predictions for the process $\mu^{\pm}e^-\rightarrow\mu^{\pm}e^-$, where for the first time an all-order resummation of soft and soft-collinear logarithms has been performed. Further, we match this resummation with the complete next-to-leading and the dominant next-to-next-to-leading higher-order corrections. We find that the resummation has a dominant effect in the signal region, while the systematic matching significantly reduces the perturbative uncertainty.

==> macros.tex <==
\usepackage{amsmath}
\usepackage{amssymb}

\usepackage{wrapfig}
\usepackage{xspace}
% \usepackage[dvipsnames]{xcolor}
\usepackage{graphicx}
\usepackage{setspace}
\usepackage{threeparttable}
\usepackage{relsize}
\usepackage{ifthen}
\usepackage{lineno}
\usepackage{enumerate}
\usepackage{makeidx}
\RequirePackage[T1]{fontenc}
\RequirePackage[utf8]{inputenc}
% \usepackage[breaklinks,colorlinks,urlcolor=blue,citecolor=citcolor,linkcolor=lcolor,linktoc=all]{hyperref}
\usepackage{hyperref}
% \usepackage{showidx}
\usepackage[acronym]{glossaries}
% \setlength{\parindent}{0.0in}
% \setlength{\parskip}{0.0in}

\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    citecolor=blue,
    filecolor=blue,
    urlcolor=blue
}
%%% Structuring
% \newcommand{\Vp}{\ensuremath{\vphantom{\frac{|^|}{|^|}}}}
% \newcommand{\LINE}{\underline{\hspace*{13.5cm}\hphantom{t}}\\}
% \newcommand{\comment}[2][]{\noindent\LINE{\bf{#1}: }{#2}\\\LINE}
% \newcommand{\todo}[1]{\textbf{\color{red}#1}}
% \newcommand{\didit}[1]{\textbf{\color{blue}did it (#1)}}
% \newcommand{\checked}[1]{\hfill{\textbf{\color{green}\checkmark(#1)}}}
% % \newcommand{\todo}[1]{\fbox{\begin{minipage}{\textwidth}\textbf{#1}\end{minipage}}}
% \newcommand{\didit}[1]{\textbf{\underline{#1}}}
% \newcommand{\checked}[1]{\hfill{\textbf{\underline{#1}}}}
\newacronym{mc}{MC}{Monte Carlo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Maths macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_maths}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Physics macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_physics}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Section references
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_refs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Experiments / Machines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_collabs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Software names
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_codes}





==> macros_codes.tex <==
\DeclareRobustCommand{\plusplus}{\raisebox{0.2ex}{\small++}}
% == ME+PS methods ======================================
%
%
\newcommand{\MCatNLO}{M\protect\scalebox{0.8}{C}@N\protect\scalebox{0.8}{LO}\xspace}
\newcommand{\SMCatNLO}{S-M\protect\scalebox{0.8}{C}@N\protect\scalebox{0.8}{LO}\xspace}
\newcommand{\POWHEG}{P\protect\scalebox{0.8}{OWHEG}\xspace}
\newcommand{\LOPS}{LO$\otimes$PS\xspace}
\newcommand{\MCatLO}{M\protect\scalebox{0.8}{C}@L\protect\scalebox{0.8}{O}\xspace}
\newcommand{\MEC}{M\scalebox{0.8}{E}C\xspace}
\newcommand{\MEPS}{M\scalebox{0.8}{E}P\scalebox{0.8}{S}\xspace}
\newcommand{\UMEPS}{UM\scalebox{0.8}{E}P\scalebox{0.8}{S}\xspace}
\newcommand{\NLOPS}{N\scalebox{0.8}{LO}P\scalebox{0.8}{S}\xspace}
\newcommand{\NNLOPS}{NN\scalebox{0.8}{LO}P\scalebox{0.8}{S}\xspace}
\newcommand{\UNLOPS}{UN\scalebox{0.8}{LO}P\scalebox{0.8}{S}\xspace}
\newcommand{\UNNLOPS}{UNN\scalebox{0.8}{LO}P\scalebox{0.8}{S}\xspace}
\newcommand{\MENLOPS}{ME\protect\scalebox{0.8}{NLO}PS\xspace}
\newcommand{\MEPSatNLO}{M\scalebox{0.8}{E}P\scalebox{0.8}{S}@N\protect\scalebox{0.8}{LO}\xspace}
\newcommand{\MINLO}{MIN\protect\scalebox{0.8}{LO}\xspace}
%
% == LO ME codes & methods ===============================
%
%
\newcommand{\Haag}{H\protect\scalebox{0.8}{AAG}\xspace}
\newcommand{\Sarge}{S\protect\scalebox{0.8}{ARGE}\xspace}
\newcommand{\Rambo}{R\protect\scalebox{0.8}{AMBO}\xspace}
\newcommand{\Vegas}{V\protect\scalebox{0.8}{EGAS}\xspace}
\newcommand{\Alpha}{A\protect\scalebox{0.8}{LPHA}\xspace}
\newcommand{\Alpgen}{A\protect\scalebox{0.8}{LPGEN}\xspace}
\newcommand{\Madgraph}{M\protect\scalebox{0.8}{AD}G\protect\scalebox{0.8}{RAPH}\xspace}
\newcommand{\Madevent}{M\protect\scalebox{0.8}{AD}E\protect\scalebox{0.8}{VENT}\xspace}
\newcommand{\Helac}{H\protect\scalebox{0.8}{ELAC}\xspace}
\newcommand{\Phegas}{P\protect\scalebox{0.8}{HEGAS}\xspace}
\newcommand{\Whizard}{W\protect\scalebox{0.8}{HIZARD}\xspace}
\newcommand{\OmegaCode}{O\protect\scalebox{0.8}{'MEGA}\xspace}
\newcommand{\Helas}{H\protect\scalebox{0.8}{ELAS}\xspace}
\newcommand{\Calchep}{C\protect\scalebox{0.8}{ALC}H\scalebox{0.8}{EP}\xspace}
\newcommand{\Comphep}{C\protect\scalebox{0.8}{OMP}H\scalebox{0.8}{EP}\xspace}
\newcommand{\UFO}{U\scalebox{0.8}{FO}\xspace}
\newcommand{\RacoonWW}{R\scalebox{0.8}{acoonWW}\xspace}
%
% == event generators ======================================
%
%
\newcommand{\Herwig}{H\protect\scalebox{0.8}{ERWIG}\xspace}
\newcommand{\Jimmy}{J\protect\scalebox{0.8}{IMMY}\xspace}
\newcommand{\HerwigJimmy}{\Herwig/\Jimmy}
\newcommand{\HerwigSix}{\Herwig{}6\xspace}
\newcommand{\HerwigSeven}{\Herwig{}7\xspace}
\newcommand{\Herwigpp}{\Herwig{}\plusplus\xspace}
\newcommand{\Ariadne}{A\protect\scalebox{0.8}{RIADNE}\xspace}
\newcommand{\Pythia}{P\protect\scalebox{0.8}{YTHIA}\xspace}
\newcommand{\PythiaSix}{\Pythia{}6\xspace}
\newcommand{\PythiaEight}{\Pythia{}8\xspace}
\newcommand{\Vincia}{V\protect\scalebox{0.8}{INCIA}\xspace}
\newcommand{\ThePEG}{T\protect\scalebox{0.8}{he}P\protect\scalebox{0.8}{EG}\xspace}
\newcommand{\Phojet}{P\protect\scalebox{0.8}{HOJET}\xspace}
\newcommand{\Epos}{E\protect\scalebox{0.8}{POS}\xspace}
\newcommand{\MLM}{M\protect\scalebox{0.8}{LM}\xspace}
\newcommand{\kkmc}{\ensuremath{\tt KKMC}\xspace}
\newcommand{\nnlojet}{NNLO\scalebox{0.8}{JET}\xspace}
%
% == NLO matching generators ======================================
%
%
\newcommand{\aMCatNLO}{aM\protect\scalebox{0.8}{C}@N\protect\scalebox{0.8}{LO}\xspace}
\newcommand{\PowhegBox}{P\protect\scalebox{0.8}{OWHEG}B\protect\scalebox{0.8}{OX}\xspace}
%
% == Resummation codes ==================================
%
%
\newcommand{\HRes}{HR\protect\scalebox{0.8}{ES}\xspace}
\newcommand{\HqT}{H\protect\scalebox{0.8}{qT}\xspace}
\newcommand{\ResBos}{R\protect\scalebox{0.8}{ES}B\protect\scalebox{0.8}{OS}\xspace}
%
% == NLO ME tools and codes =============================
%
%
\newcommand{\HelacNLO}{H\protect\scalebox{0.8}{ELAC}-NLO\xspace}
\newcommand{\AutoTools}{A\protect\scalebox{0.8}{UTO}T\protect\scalebox{0.8}{OOLS}\xspace}
\newcommand{\CutTools}{C\protect\scalebox{0.8}{UT}T\protect\scalebox{0.8}{OOLS}\xspace}
\newcommand{\Gosam}{G\protect\scalebox{0.8}{O}S\protect\scalebox{0.8}{AM}\xspace}
\newcommand{\Samurai}{S\protect\scalebox{0.8}{AMURAI}\xspace}
\newcommand{\Collier}{C\protect\scalebox{0.8}{OLLIER}\xspace}
\newcommand{\Ninja}{N\protect\scalebox{0.8}{INJA}\xspace}
\newcommand{\BlackHat}{B\protect\scalebox{0.8}{LACK}H\protect\scalebox{0.8}{AT}\xspace}
\newcommand{\Blackhat}{B\protect\scalebox{0.8}{LACK}H\protect\scalebox{0.8}{AT}\xspace}
\newcommand{\MadLoop}{M\protect\scalebox{0.8}{AD}L\protect\scalebox{0.8}{OOP}\xspace}
\newcommand{\OpenLoops}{O\protect\scalebox{0.8}{PEN}L\protect\scalebox{0.8}{OOPS}\xspace}
\newcommand{\Recola}{R\protect\scalebox{0.8}{ECOLA}}
\newcommand{\LoopTools}{L\protect\scalebox{0.8}{OOP}T\protect\scalebox{0.8}{OOLS}\xspace}
\newcommand{\FormCalc}{F\protect\scalebox{0.8}{ORM}C\protect\scalebox{0.8}{ALC}\xspace}
\newcommand{\QCDLoop}{QCDL\protect\scalebox{0.8}{OOP}\xspace}
\newcommand{\OneLoop}{O\protect\scalebox{0.8}{NE}L\protect\scalebox{0.8}{OOP}\xspace}
\newcommand{\MCFM}{M\protect\scalebox{0.8}{C}F\protect\scalebox{0.8}{M}\xspace}
\newcommand{\Njet}{N\protect\scalebox{0.8}{JET}\xspace}
\newcommand{\NLOJETpp}{N\protect\scalebox{0.8}{LOJET++}\xspace}
\newcommand{\Jetphox}{J\protect\scalebox{0.8}{ET}P\protect\scalebox{0.8}{HOX}\xspace}
\newcommand{\Diphox}{D\protect\scalebox{0.8}{I}P\protect\scalebox{0.8}{HOX}\xspace}
\newcommand{\MadgraphNLO}{M\protect\scalebox{0.8}{adGraph\_aMC@NLO}}
%
% == Subtraction tools =====================================
%
%
\newcommand{\MadDipole}{M\protect\scalebox{0.8}{AD}D\protect\scalebox{0.8}{IPOLE}\xspace}
\newcommand{\AutoDipole}{A\protect\scalebox{0.8}{UTO}D\protect\scalebox{0.8}{IPOLE}\xspace}
\newcommand{\MadFKS}{M\protect\scalebox{0.8}{AD}FKS\xspace}
\newcommand{\Matchbox}{M\protect\scalebox{0.8}{ATCH}B\protect\scalebox{0.8}{OX}\xspace}
%
% == Sherpa stuff ====================================
%
%
\newcommand{\Sherpa}{S\protect\scalebox{0.8}{HERPA}\xspace}
\newcommand{\Comix}{C\protect\scalebox{0.8}{OMIX}\xspace}
\newcommand{\Apacic}{A\protect\scalebox{0.8}{PACIC}\xspace}
\newcommand{\Amegic}{A\protect\scalebox{0.8}{MEGIC}\xspace}
\newcommand{\CSS}{CSS\protect\scalebox{0.8}{HOWER}\xspace}
\newcommand{\Dire}{D\protect\scalebox{0.8}{IRE}\xspace}
\newcommand{\Ahadic}{A\protect\scalebox{0.8}{HADIC}\xspace}
\newcommand{\Phasic}{P\protect\scalebox{0.8}{HASIC}\xspace}
\newcommand{\Adicic}{A\protect\scalebox{0.8}{DICIC}\xspace}
\newcommand{\Hadrons}{H\protect\scalebox{0.8}{ADRONS}\xspace}
\newcommand{\Photons}{P\protect\scalebox{0.8}{HOTONS}\xspace}
%
% == event generator tuning & validation ===================
%
%
\newcommand{\HEJ}{H\protect\scalebox{0.8}{EJ}\xspace}
\newcommand{\Professor}{P\protect\scalebox{0.8}{ROFESSOR}\xspace}
\newcommand{\Rivet}{R\protect\scalebox{0.8}{IVET}\xspace}
\newcommand{\Agile}{A\protect\scalebox{0.8}{GILE}\xspace}
\newcommand{\HepData}{H\protect\scalebox{0.8}{EP}D\protect\scalebox{0.8}{ATA}\xspace}
\newcommand{\HepMC}{H\protect\scalebox{0.8}{EP}MC\xspace}
\newcommand{\HZTool}{HZT\protect\scalebox{0.8}{OOL}\xspace}
\newcommand{\xfig}{XF\protect\scalebox{0.8}{IG}}
\newcommand{\xmgrace}{xmG\protect\scalebox{0.8}{RACE}}
\newcommand{\matplotlib}{M\protect\scalebox{0.8}{AT}P\protect\scalebox{0.8}{LOT}L\protect\scalebox{0.8}{IB}\xspace}
%
% == other codes ==================================
%
%
\newcommand{\FeynRules}{F\protect\scalebox{0.8}{EYN}R\protect\scalebox{0.8}{ULES}\xspace}
\newcommand{\SpringBases}{S\protect\scalebox{0.8}{PRING/}B\protect\scalebox{0.8}{ASES}\xspace}
\newcommand{\Charybdis}{C\protect\scalebox{0.8}{HARYBDIS}\xspace}
\newcommand{\Fastjet}{F\protect\scalebox{0.8}{AST}J\protect\scalebox{0.8}{ET}\xspace}
\newcommand{\EvtGen}{E\protect\scalebox{0.8}{VT}G\protect\scalebox{0.8}{EN}\xspace}
\newcommand{\Photos}{P\protect\scalebox{0.8}{HOTOS}\xspace}
\newcommand{\Tauola}{T\protect\scalebox{0.8}{AUOLA}\xspace}
\newcommand{\FEWZ}{F\protect\scalebox{0.8}{EWZ}\xspace}
\newcommand{\Jade}{J\protect\scalebox{0.8}{ADE}\xspace}
\newcommand{\Durham}{D\protect\scalebox{0.8}{URHAM}\xspace}
%
% == PDF stuff ==================================
%
%
\newcommand{\LHAPDF}{L\protect\scalebox{0.8}{HAPDF}\xspace}
\newcommand{\lostar}{\ensuremath{\text{LO}*}\xspace}
\newcommand{\cteq}[1]{\ensuremath{\text{CTEQ#1}}\xspace}
%
% == programming languages ==================================
%
%
\newcommand{\cpp}{C\plusplus\xspace}
\newcommand{\fortran}{F\scalebox{0.8}{ORTRAN}\xspace}
\newcommand{\python}{P\scalebox{0.8}{YTHON}\xspace}



==> macros_collabs.tex <==
\newcommand\fnal{F\scalebox{0.8}{NAL}\xspace}

\newcommand\tevatron{T\protect\scalebox{0.8}{EVATRON}\xspace}
\newcommand\Tevatron{\protect\tevatron}
\newcommand\runi{Run-\textsmaller{I}\xspace}
\newcommand\runii{Run-\textsmaller{II}\xspace}
\newcommand\runiia{Run-\textsmaller{II}a\xspace}
\newcommand\runiib{Run-\textsmaller{II}b\xspace}
\newcommand\cdf{CDF\xspace}
\newcommand\CDF{\cdf}
\newcommand\dzero{D\O\xspace}
\newcommand{\DO}{\dzero}

\newcommand\cern{C\scalebox{0.8}{ERN}\xspace}

\newcommand\babar{B\scalebox{0.8}{ABAR}\xspace}
\newcommand\lep{L\scalebox{0.8}{EP}\xspace}
\newcommand\lepi{L\scalebox{0.8}{EP}~1\xspace}
\newcommand\LEP{\lep}
\newcommand\LEPI{\lepi}
\newcommand\HERA{H\scalebox{0.8}{ERA}\xspace}
\newcommand\lepii{L\scalebox{0.8}{EP}~2\xspace}
\newcommand\ALEPH{A\scalebox{0.8}{LEPH}\xspace}
\newcommand\delphi{D\scalebox{0.8}{ELPHI}\xspace}
\newcommand\DELPHI{\delphi}
\newcommand\OPAL{\opal}
\newcommand\opal{O\scalebox{0.8}{PAL}\xspace}
\newcommand\Delphi{\delphi}
\newcommand\lthree{L3\xspace}
\newcommand\lhc{L\protect\scalebox{0.8}{HC}\xspace}
\newcommand\LHC{L\protect\scalebox{0.8}{HC}\xspace}
\newcommand\ATLAS{\atlas}
\newcommand\atlas{A\protect\scalebox{0.8}{TLAS}\xspace}
\newcommand\CMS{\cms}
\newcommand\cms{C\protect\scalebox{0.8}{MS}\xspace}
\newcommand\TOTEM{\totem}
\newcommand\totem{T\protect\scalebox{0.8}{OTEM}\xspace}
\newcommand\ALICE{\alice}
\newcommand\alice{A\protect\scalebox{0.8}{LICE}\xspace}
\newcommand\LHCb{\lhcb}
\newcommand\lhcb{L\scalebox{0.8}{HC}B\xspace}

\newcommand\rhic{R\scalebox{0.8}{HIC}\xspace}
\newcommand\SLD{S\scalebox{0.8}{LD}\xspace}
\newcommand\SLC{S\scalebox{0.8}{LC}\xspace}

\newcommand\JADE{J\scalebox{0.8}{ADE}\xspace}
\newcommand\hera{H\scalebox{0.8}{ERA}\xspace}
\newcommand\hone{H1\xspace}
\newcommand\zeus{Z\scalebox{0.8}{EUS}\xspace}

\newcommand\WMAP{W\scalebox{0.8}{MAP}\xspace}
\newcommand\PLANCK{P\scalebox{0.8}{LANCK}\xspace}
\newcommand\sld{SLD\xspace}

\newcommand\mcnet{MCnet\xspace}
\newcommand\pdg{PDG\xspace}
\newcommand\PDG{PDG\xspace}
\newcommand\spires{SPIRES\xspace}



==> macros_maths.tex <==
%= definitions ====================================
\newcommand{\done}{{\mathrm d}}
\newcommand{\ddone}{{\mathrm d}}
\newcommand{\dtwo}{{\mathrm d}^2}
% \newcommand{\dd}[1]{\ensuremath{d#111111}}
\newcommand{\dthree}{{\mathrm d}^3}
\newcommand{\dfour}{{\mathrm d}^4}
\newcommand{\dD}{{\mathrm d}^D}
% \newcommand{\order}{\ensuremath{\mathcal{O}}}
% \newcommand{\Order}{\ensuremath{\mathcal{O}}}
\newcommand{\oforder}[1]{\ensuremath{\mathcal{O}\left(#1 \right)}\xspace}
\newcommand{\oforderprag}[1]{\ensuremath{\mathcal{O}\left( #1 \right)_{\text{Prag}}}\xspace}
\newcommand{\dimepsilon}{\ensuremath{\varepsilon}}
\newcommand{\Li}{\mathrm{Li}}
\newcommand{\DiLi}{\ensuremath{\mathrm{Li}_2}\xspace}
\newcommand{\NGW}{N_\text{GW}}

\newcommand{\im}{\imath}
\newcommand{\jm}{\jmath}

%\newcommand{\abs}[1]{\left| #1\right|}   % conflicts with commath
\newcommand{\rbr}[1]{\left( #1\right)}
\newcommand{\abr}[1]{\langle #1\rangle}
%\newcommand{\cbr}[1]{\left\{ #1\right\}} % conflicts with commath
%\newcommand{\sbr}[1]{\left[ #1\right]}   % conflicts with commath

\newcommand{\args}[1]{\{\vec{#1}\}}
\newcommand{\argc}[2]{\{\vec{#1}\}_{\mathrm{#2}}}


\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand{\dst}{\displaystyle}
\newcommand{\sst}{\scriptstyle}

\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\nnb}{\nonumber}

\newcommand\beqn{\bea}
\newcommand\eeqn{\eea}
\newcommand\nn{\nnb}

\newcommand{\bs}{\begin{split}}
\newcommand{\es}{\end{split}}

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\bac}{\begin{array}{c}}
\newcommand{\bacc}{\begin{array}{cc}}
\newcommand{\ea}{\end{array}}

\newcommand{\mellin}[2]{\ensuremath{\mathbf{M}_{#1}\left[#2\right]}}
%\newcommand{\cal}[1]{\mathcal{#1}}
\newcommand{\BRA}[1]{\langle#1|}
\newcommand{\KET}[1]{|#1]}
%\newcommand{\spa}[2]{\langle#1\,#2\rangle}
%\newcommand{\spb}[2]{[#1\,#2]}
\def\spa#1.#2{\langle#1\,#2\rangle}
\def\spb#1.#2{[#1\,#2]}
\newcommand\slsh{\rlap{$\;\!\!\not$}}     % Feynman slash
\newcommand{\slashit}[1]{\ensuremath{{#1}\!\!/}}
\renewcommand\Re{\operatorname{\mathfrak{Re}}}
\renewcommand\Im{\operatorname{\mathfrak{Im}}}
\newcommand\Disc[1]{\operatorname{\mathfrak{Disc}}[#1]}
\def\parx{\frac{\rm d}{{\rm d}x}}
\def\pary{\frac{\rm d}{{\rm d}\vec y}}
\def\d{{\rm d}}
\def\dy{\rd y}
\def\dx{\rd x}
\def\eps{\varepsilon}
\def\MONC{\ensuremath{\mathrm{MC}}\xspace}
\def\TH{\ensuremath{\mathrm{TH}}\xspace}
\def\QCD{\ensuremath{\mathrm{QCD}}\xspace}
\def\mix{\ensuremath{\mathrm{mix}}\xspace}
\def\EW{\ensuremath{\mathrm{EW}}\xspace}
\def\PDF{\ensuremath{\mathrm{PDF}}\xspace}
\def\PDFs{\ensuremath{\mathrm{PDFs}}\xspace}
\def\siv{\ensuremath{\sigma^{(V)}}\xspace}
\def\siva{\ensuremath{\sigma^{(V_1)}}\xspace}
\def\sivb{\ensuremath{\sigma^{(V_2)}}\xspace}
\def\hatsiv{\ensuremath{\hat\sigma^{(V)}}\xspace}
\def\kv{\ensuremath{K^{(V)}}\xspace}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "sherpa"
%%% End:


==> macros_physics.tex <==

%%%% units
\newcommand{\Ummeter}{\ensuremath{\mathrm{mm}}\xspace}
\newcommand{\Umeter}{\ensuremath{\mathrm{m}}\xspace}
\newcommand{\Ukmeter}{\ensuremath{\mathrm{km}}\xspace}
\newcommand{\Ufermi}{\ensuremath{\mathrm{fm}}\xspace}
\newcommand{\Umb}{\ensuremath{\mathrm{mb}}\xspace}
\newcommand{\Uabinv}{\ensuremath{\mathrm{ab}^{-1}}\xspace}
\newcommand{\Ufbinv}{\ensuremath{\mathrm{fb}^{-1}}\xspace}
\newcommand{\Unb}{\ensuremath{\mathrm{nb}}\xspace}
\newcommand{\Upb}{\ensuremath{\mathrm{pb}}\xspace}
\newcommand{\Mpb}{\ensuremath{\mathrm{\mu b}}\xspace}
\newcommand{\UMeV}{\ensuremath{\mathrm{MeV}}\xspace}
\newcommand{\UGeV}{\ensuremath{\mathrm{GeV}}\xspace}
\newcommand{\UGeVt}{\ensuremath{\mathrm{GeV}^2}\xspace}
\newcommand{\UTeV}{\ensuremath{\mathrm{TeV}}\xspace}
\newcommand{\mrad}{\ensuremath{\mathrm{mrad}}\xspace}
\newcommand{\rad}{\ensuremath{\mathrm{rad}}\xspace}

% Kinematical quantities
\newcommand{\Ecm}{\ensuremath{E_{\mathrm{c.m.}}}\xspace}
\newcommand{\hatEcm}{\ensuremath{\hat{E}_{\mathrm{c.m.}}}\xspace}
\newcommand{\kt}{\ensuremath{k_T}\xspace}
\newcommand{\kT}{\kt}
\newcommand{\kperp}{\kt}
\newcommand{\sqrts}{\ensuremath{\sqrt{s}}\xspace}
\newcommand{\sqrtsp}{\ensuremath{\sqrt{s^\prime}}\xspace}
\newcommand{\hsqrts}{\ensuremath{\frac{\sqrt{s}}{2}}\xspace}
\newcommand{\shat}{\ensuremath{\hat{s}}\xspace}
\newcommand{\mt}{\ensuremath{m_T}\xspace}
\newcommand{\pt}{\ensuremath{p_T}\xspace}
\newcommand{\HT}{\ensuremath{H_T}\xspace}
\newcommand{\ptzero}{\ensuremath{p_{T,0}}\xspace}
\newcommand{\ptmin}{\ensuremath{p_{T,\mathrm{min}}}\xspace}
\newcommand{\Etmiss}{\ensuremath{E\!\!\!\!/_T}\xspace}
\newcommand{\mT}{\mt}
\newcommand{\pT}{\pt}
\newcommand{\QT}{\ensuremath{Q_T}}
\newcommand{\pperp}{\pt}
% variants of pT that can take an argument
\newcommand{\mPerp}[1]{\ensuremath{m_{T #1}}\xspace}
\newcommand{\pPerp}[1]{\ensuremath{p_{T #1}}\xspace}

%%%% Reactions
\newcommand{\pp}{\ensuremath{pp}\xspace}
\newcommand{\ww}{\ensuremath{W^+W^-}\xspace}
\newcommand{\zh}{\ensuremath{ZH}\xspace}
\newcommand{\ppbar}{\ensuremath{p\bar{p}}\xspace}
\newcommand{\epluseminus}{\ensuremath{e^+ e^-}\xspace}
\newcommand{\ee}{\epluseminus}
\newcommand{\mumu}{\ensuremath{\mu^+\mu^-}\xspace}
\newcommand{\tautau}{\ensuremath{\tau^+\tau^-}\xspace}
\newcommand{\eeee}{\ensuremath{\ee \rightarrow \ee}\xspace}
\newcommand{\eemumu}{\ensuremath{\ee \rightarrow \mumu}\xspace}
\newcommand{\eezh}{\ensuremath{\ee \rightarrow \zh}\xspace}
\newcommand{\eeww}{\ensuremath{\ee \rightarrow \ww}\xspace}
\newcommand{\eeaz}{\ensuremath{\ee \rightarrow \gamma^* Z}\xspace}
\newcommand{\eevv}{\ensuremath{\ee \rightarrow VV}\xspace}
\newcommand{\eewwfusion}{\ensuremath{\ee \rightarrow (\ww\rightarrow H)\nu\bar{\nu}}\xspace}
\newcommand{\eetautau}{\ensuremath{\ee \rightarrow \tautau}\xspace}
\newcommand{\ep}{\ensuremath{e^\pm p}\xspace}
\newcommand{\ffbar}{\ensuremath{f \bar{f}}}
\newcommand{\eeffbar}{\ensuremath{\ee \rightarrow \ffbar}\xspace}
\newcommand{\eeffbarng}{\ensuremath{\ee \rightarrow \ffbar + n\gamma}\xspace}
\newcommand{\eeWW}{\ensuremath{\ee \rightarrow W^+W^-}\xspace}
\newcommand{\eefour}{\ensuremath{\ee \rightarro 4f}\xspace}
\newcommand{\eeWWfour}{\ensuremath{\eeWW \rightarrow 4f}\xspace}
\newcommand{\eeWWfourA}{\ensuremath{\eeWW \rightarrow 4f + \gamma}\xspace}
\newcommand{\ttbar}{\ensuremath{t\bar t}\xspace}
\def\wpl{\ensuremath{\ell^+\nu_\ell}}
\def\wml{\ensuremath{\ell^-\bar\nu_\ell}}
\def\zll{\ensuremath{\ell^+\ell^-}}
\def\znn{\ensuremath{\nu\bar\nu}}
\def\emup{\ensuremath{\mu^+e^-\rightarrow\mu^+e^-}\xspace}
\def\emum{\ensuremath{\mu^-e^-\rightarrow\mu^-e^-}\xspace}
\def\emupm{\ensuremath{\mu^{\pm}e^-\rightarrow\mu^{\pm}e^-}\xspace}
\def\tee{\ensuremath{t_{e^-e^-}}\xspace}
%%%% Particles and their properties
%% bosons
\DeclareRobustCommand{\PH}{{\ensuremath{h}}}
\DeclareRobustCommand{\PZ}{{\ensuremath{\mathrm{Z}}}}
\DeclareRobustCommand{\PW}{{\ensuremath{\mathrm{W}}}}
\DeclareRobustCommand{\PWpm}{{\ensuremath{\mathrm{W}^{\pm}}}}
%% leptons
\DeclareRobustCommand{\Pl}{{\ensuremath{\ell}}}
\DeclareRobustCommand{\Pal}{{\ensuremath{\bar{\ell}}}}
\DeclareRobustCommand{\Plp}{{\ensuremath{\ell^+}}}
\DeclareRobustCommand{\Plm}{{\ensuremath{\ell^-}}}
%% nucleons
\DeclareRobustCommand{\Pp}{{\ensuremath{\mathrm{p}}}}
%% masses
\newcommand{\MW}{\ensuremath{m_W}}
\newcommand{\MH}{\ensuremath{m_H}}
\newcommand{\MZ}{\ensuremath{m_Z}}
\newcommand{\MT}{\ensuremath{m_t}}
\newcommand{\MB}{\ensuremath{m_b}}
\newcommand{\MC}{\ensuremath{m_c}}
\newcommand{\MS}{\ensuremath{m_s}}
\newcommand{\MD}{\ensuremath{m_d}}
\newcommand{\MU}{\ensuremath{m_u}}
\newcommand{\Mtau}{\ensuremath{m_\tau}}
\newcommand{\GW}{\ensuremath{\Gamma_W}}
\newcommand{\GZ}{\ensuremath{\Gamma_Z}}
\newcommand{\GH}{\ensuremath{\Gamma_H}}
\newcommand{\GT}{\ensuremath{\Gamma_t}}

\newcommand{\SU}[1]{\ensuremath{\text{SU}(#1)}}
\newcommand{\su}[1]{\SU{#1}}

%%%% Couplings
\newcommand{\MSbar}{\ensuremath{\overline{\mathrm{MS}}}}
\newcommand{\llalphaps}{\ensuremath{\alpha_{\text{s,PS}}}\xspace}
\newcommand{\alphaS}{\ensuremath{\alpha_\text{s}}\xspace}
\newcommand{\alphaSn}[1]{\ensuremath{\alpha^#1_\text{s}}\xspace}
\newcommand{\alphaW}{\ensuremath{\alpha_\text{w}}\xspace}
\newcommand{\alphaQED}{\ensuremath{\alpha_\text{QED}}\xspace}
\newcommand{\Nc}{\ensuremath{N_c}\xspace}
\newcommand{\nf}{\ensuremath{n_f}}
\newcommand{\CF}{\ensuremath{C_F}}
\newcommand{\CA}{\ensuremath{C_A}}
\newcommand{\TR}{\ensuremath{T_R}}
\newcommand{\LambdaQCD}{\ensuremath{\Lambda_\text{QCD}}\xspace}
\newcommand{\gs}{\ensuremath{g_s}}
\newcommand{\gW}{\ensuremath{g_W}}
\newcommand{\gFermi}{\ensuremath{G_F}}
\newcommand{\GF}{\gFermi}
\newcommand{\sinW}{\ensuremath{\sin\theta_W}}
\newcommand{\cosW}{\ensuremath{\cos\theta_W}}
\newcommand{\sinSqW}{\ensuremath{\sin^2\theta_W}}
\newcommand{\cosSqW}{\ensuremath{\cos^2\theta_W}}
\newcommand{\BR}[1]{\ensuremath{\mathcal{BR}_{#1}}}
\newcommand{\DeltaPom}{\ensuremath{{\Delta_{\mathbf{P}}}}\xspace}
\newcommand{\DeltaHad}{\ensuremath{{\Delta \alpha_{\text{had}}}(t)}\xspace}
\newcommand{\ahlo}{\ensuremath{\alpha_\mu^\text{HLO}}\xspace}


\newcommand{\pdf}[2]{\ensuremath{f_{#2/#1}}}
\newcommand{\ff}[2]{\ensuremath{D_{#2/#1}}}
\newcommand{\muR}{\ensuremath{\mu_R}}
\newcommand{\muF}{\ensuremath{\mu_F}}
\newcommand{\muQ}{\ensuremath{\mu_Q}}
\newcommand{\Ecms}{\ensuremath{E_\mathrm{cms}}}
\newcommand{\mucut}{\ensuremath{\mu_{Q_\mathrm{cut}}}}
\newcommand{\ycut}{\ensuremath{y_\mathrm{cut}}}
\newcommand{\Qcut}{\ensuremath{Q_\mathrm{cut}}}
\newcommand{\QcutSq}{\ensuremath{Q_\mathrm{cut}^2}}
\newcommand{\Qiso}{\ensuremath{Q_\mathrm{iso}}}
\newcommand{\tcut}{\ensuremath{t_\mathrm{c}}}
\newcommand{\nmax}{\ensuremath{N_\mathrm{max}}}
\newcommand{\nmin}{\ensuremath{N_\mathrm{min}}}
\newcommand{\tnmax}{\ensuremath{t_\nmax}}
\newcommand{\tcutQED}{\ensuremath{t_{\mathrm{c},\mathrm{(QED)}}}}
\newcommand{\alphacut}{\ensuremath{\alpha_{\mathrm{cut}}}}

%%%% Bits of calculations
\newcommand{\tFFDipole}[3]{\ensuremath{{\tilde{\mathcal{D}}_{#1#2;#3}}}}
\newcommand{\Dipole}{\ensuremath{{\mathcal{D}}}}
\newcommand{\tDipole}{\ensuremath{\tilde{\mathcal{D}}}}
\newcommand{\IntDip}{\ensuremath{{\mathcal{I}^{(\mathcal{D})}}}}
\newcommand{\IntDipole}[2]{\ensuremath{{\mathcal{I}^{(\mathcal{D})}_{#1;#2}}}}
\newcommand{\FFDipole}[3]{\ensuremath{{\mathcal{D}_{#1#2;#3}}}}
\newcommand{\FIDipole}[3]{\ensuremath{{\mathcal{D}_{#1#2}^{#3}}}}
\newcommand{\IFDipole}[3]{\ensuremath{{\mathcal{D}^{#1#2}_{#3}}}}
\newcommand{\IIDipole}[3]{\ensuremath{{\mathcal{D}^{#1#2;#3}}}}
\newcommand{\DipOp}[1]{\ensuremath{{\mathbf{D}}(#1)}}
\newcommand{\IntDipOp}[2]{\ensuremath{{\mathbf{I}}(#1;\,#2)}}
\newcommand{\IntDipOpFF}[2]{\ensuremath{{\mathbf{I}}_{FF}(#1;\,#2)}}
\newcommand{\IntDipOpFI}[2]{\ensuremath{{\mathbf{I}}_{FI}(#1;\,#2)}}
\newcommand{\IntDipOpIF}[2]{\ensuremath{{\mathbf{I}}_{IF}(#1;\,#2)}}
\newcommand{\IntDipOpII}[2]{\ensuremath{{\mathbf{I}}_{II}(#1;\,#2)}}
\newcommand{\Eikonal}[4]{\ensuremath{{\mathcal{W}(#1,\,#2;\,#3,\,#4)}}}
\newcommand{\Eik}{\ensuremath{{\mathrm{W}}}}
\newcommand{\Ampl}{\ensuremath{{\mathcal{A}}}}
\newcommand{\Prob}{\ensuremath{{\mathcal{P}}}}
\newcommand{\Sub}{\ensuremath{{\mathcal{S}}}}
\newcommand{\SubKernel}{\ensuremath{\tilde{\mathcal S}}}
\newcommand{\SubKInt}{\ensuremath{\tilde{S}}}
\newcommand{\Born}{\ensuremath{{\mathcal{B}}}}
\newcommand{\Hard}{\ensuremath{{\mathcal{H}}}}
\newcommand{\Evol}[2]{\ensuremath{{\mathcal{E}_{#1}^{(#2)}}}}
\newcommand{\EvolIn}[3]{\ensuremath{{\mathcal{E}_{#1}^{(#2,<#3)}}}}
\newcommand{\bBorn}{\ensuremath{\bar{\mathcal{B}}}}
\newcommand{\tBorn}{\ensuremath{\tilde{\mathcal{B}}}}
\newcommand{\Real}{\ensuremath{{\mathcal{R}}}}
\newcommand{\Subtraction}{\ensuremath{{\mathcal{S}}}}
\newcommand{\IntSubtraction}{\ensuremath{\mathcal{I}^{(\mathcal{S})}}}
\newcommand{\RealS}{\ensuremath{{\mathcal{R}}^{(\mathrm{S})}}}
\newcommand{\RealH}{\ensuremath{{\mathcal{R}}^{(\mathrm{H})}}}
\newcommand{\Virtual}{\ensuremath{{\mathcal{V}}}}
\newcommand{\Kernel}{\ensuremath{\mathcal{K}}}
\newcommand{\KernelIn}[1]{\ensuremath{\Kernel^{<#1}}}
\newcommand{\KernelOut}[1]{\ensuremath{\Kernel^{\ge#1}}}
\newcommand{\BornPS}{\ensuremath{\Phi_{{\mathcal{B}}}}}
\newcommand{\RealPS}{\ensuremath{\Phi_{{\mathcal{R}}}}}
\newcommand{\OnePS}{\ensuremath{\Phi_{1}}}
\newcommand{\PS}[1]{\ensuremath{\Phi_{#1}}}
\newcommand{\LO}{\ensuremath{\mathrm{LO}}\xspace}
\newcommand{\NLO}{\ensuremath{\mathrm{NLO}}\xspace}
\newcommand{\NLOQCD}{\ensuremath{\mathrm{NLO_{QCD}}}\xspace}
\newcommand{\NNLOQCD}{\ensuremath{\mathrm{NNLO_{QCD}}}\xspace}
\newcommand{\NLOEW}{\ensuremath{\mathrm{NLO_{EW}}}\xspace}
\newcommand{\NNLOEW}{\ensuremath{\mathrm{NNLO_{EW}}}\xspace}
\newcommand{\NNLO}{\ensuremath{\mathrm{NNLO}}\xspace}
\newcommand{\NNNLO}{\ensuremath{\mathrm{N^3LO}}\xspace}
\newcommand{\Me}{\ensuremath{\mathcal{M}}}
\newcommand{\ME}[1]{\ensuremath{\mathcal{M}^{({#1})}}}
\newcommand{\MEstar}[1]{\ensuremath{\mathcal{M}^{*({#1})}}}
\newcommand{\Splitting}{\ensuremath{\mathcal{P}}}
\newcommand{\splitting}[2]{\ensuremath{\mathcal{P}_{#1#2}}}
\newcommand{\Nsplitting}[2]{\ensuremath{\hat{\mathcal{P}}_{#1#2}}}
\newcommand{\helsum}{\ensuremath{\bar\Sigma_{\mathrm hel.}}}
\newcommand{\prefD}{\ensuremath{\mu^{4-D}}}
\newcommand{\LoopD}[1]{\ensuremath{\frac{\dD{#1}}{(2\pi)^D}}}
% \newcommand{\Tr}[1]{\ensuremath{\mathrm{Tr}\left[#1\right]}}
\newcommand{\sla}[1]{\ensuremath{{#1\kern-0.45em/}}}
\newcommand{\betatilde}[2]{\ensuremath{\tilde{\beta}_{#1}^{#2}}\xspace}
\newcommand{\betatildeK}[3]{\ensuremath{\tilde{\beta}_{#1}^{#2}}\left(#3\right)\xspace}
\newcommand{\bV}{{\bf V}}

\newcommand{\lagrange}{\ensuremath{\mathcal{L}}}
\newcommand{\lumi}{\ensuremath{\mathcal{L}}}
\newcommand{\sigtot}{\ensuremath{\sigma_{\mathrm{tot}}}}
\newcommand{\sigeff}{\ensuremath{\sigma_{\mathrm{eff}}}}
\newcommand{\sigel}{\ensuremath{\sigma_{\mathrm{el}}}}
\newcommand{\siginel}{\ensuremath{\sigma_{\mathrm{inel}}}}
\newcommand{\BRatio}[1]{\ensuremath{\mathrm{BR}_{#1}}}
\newcommand{\Rate}[1]{\ensuremath{\mathfrak{R}_{#1}}}

\newcommand{\aCDR}{\ensuremath{a^{\mathrm{CDR}}}}

\newcommand{\antikT}[1]{anti-$k_T$~($D=0.#1$)}
\newcommand{\midpoint}{M\protect\scalebox{0.8}{ID}P\protect\scalebox{0.8}{OINT}\xspace}

\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}


\newcommand{\gmu}{\ensuremath{\gamma^\mu}}
\newcommand{\gnu}{\gamma^\nu}
\newcommand{\umu}{^\mu}
\newcommand{\dmu}{_\mu}
\newcommand{\unu}{^\nu}
\newcommand{\dnu}{_\nu}
\newcommand{\umunu}{^{\mu\nu}}
\newcommand{\dmunu}{_{\mu\nu}}

\newcommand{\eik}[1]{\ensuremath{\tilde{S}\left(k_{#1}\right)}}
\newcommand{\eikK}{\ensuremath{\tilde{S}\left(k\right)}}
\newcommand{\eiki}{\ensuremath{\tilde{S}(k_i)}}
\newcommand{\eikbar}{\ensuremath{\tilde{S}(\bar{k}_i)}}
\newcommand{\sigmaborn}{\ensuremath{\sigma_{\text{Born}}}}
\newcommand{\gammabar}{\ensuremath{\bar{\gamma}}}
\newcommand{\bbeta}{\ensuremath{\bar{\beta}}}
\def\born{{\rm Born}}

\newcommand{\deltaqcd}[1]{\ensuremath{\delta^{(#1)} K^{(V)}_{N^kLO}}\xspace}
\newcommand{\yfslo}{\ensuremath{\mathrm{YFS}_{\mathbf{LO}}}\xspace}
\newcommand{\yfsnlo}{\ensuremath{\mathrm{YFS}_{\mathbf{NLO}}}\xspace}
\newcommand{\yfsnnlo}{\ensuremath{\mathrm{YFS}_{\mathbf{nNLO}}}\xspace}
\newcommand{\Deltayfs}[1]{\ensuremath{\Delta \mathrm{YFS}_{\mathbf{#1}}\xspace}}
\newcommand{\eeffbarDiagram}{\feynmandiagram{
  i1 [particle=\(e^{-}\)] -- [fermion] a --  [fermion] i2 [particle=\(e^{+}\)],
  a -- [photon, edge label=\(\gamma\), momentum'=\(k\)] b,
  % f1 [particle=\(\mu^{+}\)] -- [fermion] b -- [fermion] f2 [particle=\(\mu^{-}\)],
  };
}


==> macros_refs.tex <==
\newcommand{\EqRef}[1]{Eq.~\eqref{#1}\xspace}
\newcommand{\EqsRef}[2]{Eqs.~\eqref{#1} -- \eqref{#2}\xspace}
\newcommand{\EqRefs}[2]{Eqs.~\eqref{#1} and \eqref{#2}\xspace}
\newcommand{\EqRefsT}[3]{Eqs.~\eqref{#1}, \eqref{#2} and \eqref{#3}\xspace}
\newcommand{\PageRef}[1]{page~\pageref{#1}\xspace}
\newcommand{\PagesRef}[2]{pages~\pageref{#1} -- \pageref{#2}\xspace}
\newcommand{\ChapRef}[1]{Chapter~\ref{#1}\xspace}
\newcommand{\ChapRefs}[2]{Chapters~\ref{#1} and \ref{#2}\xspace}
\newcommand{\ChapsRef}[2]{Chapters~\ref{#1} -- \ref{#2}\xspace}
\newcommand{\SecRef}[1]{Section~\ref{#1}\xspace}
\newcommand{\SecRefs}[2]{Sections~\ref{#1} and \ref{#2}\xspace}
\newcommand{\SecsRef}[2]{Sections~\ref{#1} -- \ref{#2}\xspace}
\newcommand{\AppRef}[1]{Appendix~\ref{#1}\xspace}
\newcommand{\AppRefs}[2]{Appendics~\ref{#1} and \ref{#2}\xspace}
\newcommand{\FigRef}[1]{Fig.~\ref{#1}\xspace}
\newcommand{\FigRefs}[2]{Figs.~\ref{#1} and~\ref{#2}\xspace}
\newcommand{\FigsRef}[2]{Figs.~\ref{#1} -- \ref{#2}\xspace}
\newcommand{\TabRef}[1]{Tab.~\ref{#1}\xspace}
\newcommand{\TabsRef}[1]{Tabs.~\ref{#1}\xspace}
\newcommand{\mycaption}[3]{\parbox{.8\textwidth}{\caption[#1]{#2\label{#3}}}}
\newcommand{\mycaptionwide}[3]{\parbox{\textwidth}{\caption[#1]{#2\label{#3}}}}
\newcommand{\mycaptionhalf}[3]{\parbox{.4\textwidth}{\caption[#1]{#2\label{#3}}}}
\newcommand{\eg}{{\itshape e.g.}\xspace}
\newcommand{\ie}{{\itshape i.e.}\xspace}
\newcommand{\cf}{{\itshape cf.}\xspace}
\newcommand{\etc}{{\itshape etc.}\xspace}

\newcommand{\gloss}[2]{{\bf #1:} #2}

